Dark Energy Survey's Observation Strategy, Tactics, and Exposure Scheduler

The Dark Energy Survey is a stage III dark energy experiment, performing an optical imaging survey to measure cosmological equation of state parameters using four independent methods. The scope and complexity of the survey introduced complex strategic and tactical scheduling problems that needed to be addressed. We begin with an overview of the process used to develop DES strategy and tactics, from the inception of the project, to task forces that studied and developed strategy changes over the course of the survey, to the nightly pre-observing meeting in which immediate tactical issues were addressed. We then summarize the strategic choices made for each sub-survey, including metrics, scheduling considerations, choice of time domain fields and their sequences of exposures, and wide survey footprint and pointing layout choices. We go on to describe the detailed process that determined which specific exposures were taken at which specific times. We give a chronology of the strategic and tactical peculiarities of each year of observing, including the proposal and execution of a sixth year. We give an overview of obstac, the implementation of the DES scheduler used to simulate and evaluate strategic and tactical options, and automate exposure scheduling; and describe developments in obstac for use after DES. Appendices describe further details of data quality evaluation, tau, and t_eff; airmass calculation; and modeling of the seeing and sky brightness. The significant corpus of DES data indicates that the simple scaling relations for seeing as a function of wavelength and airmass derived from the Kolmogorov turbulence model work adequately for exposure planning purposes: deviations from these relations are modest in comparison with short time-scale seeing variations.

==> architecture.tex <==
\section{\obstac architecture details}

\begin{figure*}
\centering
\resizebox{0.9\linewidth}{!}{\input{circ_class_diagram.latex}}
\caption{\label{fig:circclassdiag}
Class diagram showing interchangeable elements of \texttt{ObsCircumstance}.}
\end{figure*}



==> lessons.tex <==
\section{Lessons learned}

\todo[inline]{make fewer assumptions in the database}


==> requirements.tex <==
\section{Requirements}

\subsection{\emph{De Jure} requirements}

\cite{annis_decam_2005} is the official functional requirements document for
\obstac. It provides the following requirements\footnote{The numbering is
not official, but added for convenient reference here. The text itself
is a direct quote from \cite{annis_decam_2005}}:

\begin{quote}
\begin{enumerate}
\item \obstac must be capable of being overridden by the on-site astronomer.
\item \obstac must be aware of relevant observatory states such as
weather, twilight, and moon-rise. Likewise, \obstac must be aware of
instrumental states such as exposure complete and of survey status
such as tiles completed.
\item \obstac must allow for simple scripting of a given series of
exposures. This the primary usage case for community astronomers
and a good general purpose dither pattern should be provided.
\item \obstac must allow for scripting of algorithms that allow for
efficient choice of the next tile to observe and generally the
next observation to take. A typical DES algorithm would take as
inputs: 1) time, to compute moon position and twilight status 2)
survey status, in the form of tiles observed. It would locate
candidate tiles from the survey status information, and compute
airmasses for the candidates. Given this information it would
compute a metric for each candidate and then choose the best tile
to observe.
\item \obstac must send to the OCS all the information needed for the
observation: R.A., declination, exposure time, filter.
\item Depending on weather, there may be other tactical plans to
follow. It will be up to the on-site astronomer to choose the
appropriate plan.
\item Likewise, there may be calibration plans to follow. For example,
we imagine pointing at a resolved local galaxy every night for
photometric and astrometric calibrations. The whole sequence of
observations would constitute a tactical plan, to be chosen by the
on-site astronomer.
\item \obstac, once started with a plan, will continue generating
observations until there are no more valid observations to take
(in the context of the plan, i.e., the sun has come up, or the
calibration sequence is completed) or overridden by the on-site
astronomer.
\item \obstac will update its survey status information during the night
automatically. The survey status information must be able to be
reloaded given, for example, a list of tiles completed by data
reduction.
\end{enumerate}
\end{quote}

These requirements, last revised in 2005, are both general and out of
date. In particular, changes in the SISPI architecture have resulted in
other SISPI components performing the function described in
requirements 3, 7, and 9 being performed by other SISPI components; in
practice, these are no longer requirements on \obstac, although they
are requirements on the SISPI system as a whole.

\subsection{\emph{De facto} requirements}

In addition to the \emph{de jure} requirements, a number of \emph{de facto}
requirements are imposed on \obstac by the SISPI architecture,
interfaces to other systems, survey strategy, and the use cases
\obstac needs to support. *The \emph{de facto} requirements described here
have no official standing, and are a representation only of the
project's needs as perceived by the \obstac developer.*

\obstac's requirements may be divided into several broad categories:
these specific for each use case, and those in common to all use
cases. The requirements specific to each use case primarily concern
the interfaces between \obstac and external systems, either SISPI or
the user. Those in common to all use cases concern \obstac's central
function: the selection of exposures or sequences of exposures based
on DES survey strategy.

The central requirement, common to all use cases, is that:

\begin{enumerate}
\item \obstac must select exposures that implement the DES survey
strategy, as set by survey management based on recommendation from
the Survey Strategy Taskforce (SSTF).
\end{enumerate}

The following requirements are imposed by the simulation use case:

\begin{enumerate}
\setcounter{enumi}{1}
\item A user must be able to initiate a simulation.
\item The simulation must produce a data set providing at least the
following data on each exposure: exposure start time and date,
R.A., declination, filter, exposure time, simulated seeing,
simulated cloud cover, simulated sky brightness, and whether the
simulation itself accepted the exposure as being "good" data.
\item The simulation must provide the exposure data set in a format that
the survey scientist and other members of the SSTF find convenient.
\item The simulation must model the time between exposures based on a
model of slew time time and CCD readout time.
\item The simulation must model the seeing based on a model derived from
historical DIMM data from CTIO.
\item The simulation must model the cloud cover based on historical
cloud cover data recorded at CTIO for different years.
\end{enumerate}

The following requirements are imposed by the observing operations use
case:

\begin{enumerate}
\setcounter{enumi}{7}
\item \obstac must be runnable as one or more SISPI applications, to be
started by the SISPI Architect.
\item \obstac must collect the data it requires for exposures select
through queries to the SISPI postgresql database.
\item An \texttt{enable} command sent to an \obstac application in the
\texttt{AutoObs} SISPI role must enable \obstac, causing it to respond
to \texttt{UpdateQueue} events by selecting exposures and sending
corresponding PML \texttt{add} messages to the SISPI application filling
the OCS role.
\item A \texttt{disable} command set to an \obstac application in the
\texttt{AutoObs} SISPI role must disable \obstac, causing it not to add
exposures to the queue.
\end{enumerate}
